Appraisal of a Random Bit Generator Utilizing Smartphone Sensors as Entropy Source

We aim to access entropy sources available within smartphones in order to construct and evaluate a random number generator which is competitive in comparison with existing and proven random number generators. A prototype utilizing the herein proposed algorithm shall generate data that can be tested against the Statistical Test Suit provided by NIST. Although our initial intention of using cosmic radiation failed, we were able to extract randomness from incoming video and audio sources. We found that it is possible to access these sources of entropy utilizing sensors from smartphones resulting in 15 out of 15 successful passed tests within the Statistical Test Suit. We also found that wrong methods of sensor data collection using our prototype eventually generates weak random numbers and fails NIST's Statistical Test Suit. Finally, we suggest that in order to reach the initial goal of providing a smartphone-based true nondeterministic random number generator the detection of muons shall be researched.

==> chapters/99_acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Acronyms}
\label{chap:acronyms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Which one will be the longest ...?
% ABCDE --> \begin{acronym}[ABCDE]
\footnotesize
\begin{acronym}[ABCDE]
  \acro{BSI}{Backside Illuminated}
  \acro{CCD}{Charge Coupled Device}
  \acro{CERN}{Conseil Europ\'{e}en pour la Recherche Nucl\'{e}aire}
  \acro{CMOS}{Complementary Metal Oxide Semiconductor}
  \acro{DRBG}{Deterministic Random Bit Generator}
  \acro{DRNG}{Deterministic Random Number Generator}
  \acro{ERBG}{Economical Random Bit Generator}
  \acro{ERNG}{Economical Random Number Generator}
  \acro{HDD}{Hard Drive Disc}
  \acro{NIST}{National Institute of Standards and Technology}
  \acro{NRBG}{Non-deterministic Random Bit Generator}
  \acro{PRNG}{Pseudo Random Number Generator}
  \acro{PBS}{Polarized Beam Splitter}
  \acro{QRNG}{Quantum Random Number Generator}
  \acro{RBG}{Random Bit Generator}
  \acro{RNG}{Random Number Generator}
  \acro{TRNG}{True Random Number Generator}



\end{acronym}
\normalsize

